Quiver description of bow varieties in general type

We provide a quiver description for Cherkis bow varieties in arbitrary type. We explain how this generalizes the construction of Nakajima quiver varieties. We give criteria for stability, non-emptiness, smoothness and discuss deformations. In the appendix, we discuss the relation between the quiver description and the original Cherkis' construction of bow varieties.

==> ex-emptiness-2.tex <==
\begin{tikzcd}
\mathbb{C}^2 \arrow[r, "C", shift left] & \mathbb{C}^5 \arrow["B^-", loop, distance=2em, in=55, out=125] \arrow[rr, "A"] \arrow[rd, "b"'] \arrow[l, "D", shift left] &                             & \mathbb{C}^2 \arrow["B^+", loop, distance=2em, in=55, out=125] \\
                                        &                                                                                                                            & \mathbb{C} \arrow[ru, "a"'] &                                                               
\end{tikzcd}
